Learning Dynamic Bayesian Networks from Data: Foundations, First Principles and Numerical Comparisons

In this paper, we present a guide to the foundations of learning Dynamic Bayesian Networks (DBNs) from data in the form of multiple samples of trajectories for some length of time. We present the formalism for a generic as well as a set of common types of DBNs for particular variable distributions. We present the analytical form of the models, with a comprehensive discussion on the interdependence between structure and weights in a DBN model and their implications for learning. Next, we give a broad overview of learning methods and describe and categorize them based on the most important statistical features, and how they treat the interplay between learning structure and weights. We give the analytical form of the likelihood and Bayesian score functions, emphasizing the distinction from the static case. We discuss functions used in optimization to enforce structural requirements. We briefly discuss more complex extensions and representations. Finally we present a set of comparisons in different settings for various distinct but representative algorithms across the variants.

==> name.tex <==
\subsection{Forecasting Prediction Accuracy}

\emph{Favorable Data Regime}

\begin{table}
    \begin{tabular}{l | c | c | c | c |}
    Data & (3,50,1) & (5,100,1) & (10,500,1) & (3,30,10) \\ \hline
    \textbf{PCMCI} & & & & \\ \hline
    \textbf{GOBNILP} & & & & \\ \hline
    \textbf{ILP (Manzour et al)} & & & & \\ \hline
    \textbf{One Shot Frequentist ILP} & & & & \\ \hline
    \textbf{GFlowNets} & & & & \\ \hline
    \textbf{GFlowNets with Parameter} & & & & \\ \hline
    \textbf{DYNOTEARS} & & & & \\ \hline
    \textbf{Greedy MC} & & & & \\ \hline
    \end{tabular}
    \caption{Model Forecasting Accuracy for the Favorable Data Regime across Algorithms}
\end{table}

\begin{table}
    \begin{tabular}{l | c | c | c | c |}
    \hline \\
    Data & (5,50,50) & (10,100,200) & (20,400,400) & (30,600,500)  \\ \hline 
    \textbf{PCMCI} & & & & \\ \hline
    \textbf{GOBNILP} & & & & \\ \hline
    \textbf{ILP (Manzour et al)} & & & & \\ \hline
    \textbf{One Shot Frequentist ILP} & & & & \\ \hline
    \textbf{GFlowNets} & & & & \\ \hline
    \textbf{GFlowNets with Parameter} & & & & \\ \hline
    \textbf{DYNOTEARS} & & & & \\ \hline
    \textbf{Greedy MC} & & & & \\ \hline
    \end{tabular}
    \caption{Model Forecasting Accuracy for the Favorable Data Regime across Algorithms}
    \end{table}


\emph{High Dimensional Regime}

\begin{table}
    \begin{tabular}{l | c | c | c | c |}
    Data & (3,10,1) & (5,20,1) & (10,50,1) & (3,5,10) \\ \hline
    \textbf{PCMCI} & & & & \\ \hline
    \textbf{GOBNILP} & & & & \\ \hline
    \textbf{ILP (Manzour et al)} & & & & \\ \hline
    \textbf{One Shot Frequentist ILP} & & & & \\ \hline
    \textbf{GFlowNets} & & & & \\ \hline
    \textbf{GFlowNets with Parameter} & & & & \\ \hline
    \textbf{DYNOTEARS} & & & & \\ \hline
    \textbf{Greedy MC} & & & & \\ \hline
    \end{tabular}
    \caption{Model Forecasting Accuracy for the High Dimensional Data Regime across Algorithms}
\end{table}

\begin{table}
    \begin{tabular}{l | c | c | c | c |}
    \hline \\
    Data & (5,10,20) & (10,20,40) & (20,40,50) & (30,60,100)  \\ \hline 
    \textbf{PCMCI} & & & & \\ \hline
    \textbf{GOBNILP} & & & & \\ \hline
    \textbf{ILP (Manzour et al)} & & & & \\ \hline
    \textbf{One Shot Frequentist ILP} & & & & \\ \hline
    \textbf{GFlowNets} & & & & \\ \hline
    \textbf{GFlowNets with Parameter} & & & & \\ \hline
    \textbf{DYNOTEARS} & & & & \\ \hline
    \textbf{Greedy MC} & & & & \\ \hline
    \end{tabular}
    \caption{Model Forecasting Accuracy for the High Dimensional Data Regime across Algorithms}
    \end{table}

==> oldnotes.tex <==


= \prod\limits_{n=1}^N \prod\limits_{t=1}^{T-1} \left[\mathbf{1}(X^{(n)}_i(t+1)=1)\sigma\left(\theta^{\bar{\mathcal{G}},i}_0+\sum\limits_{j\in dpa(i)} \theta^{\bar{\mathcal{G}},i}_{j} V_j\right) \right. \\
\qquad\left.+\mathbf{1}(X^{(n)}_i(t+1)=0)\left(1-\sigma\left(\theta^{\bar{\mathcal{G}},i}_0+\sum\limits_{j\in dpa(i)} \theta^{\bar{\mathcal{G}},i}_{j} V_j\right)\right)\right]\\
=\prod\limits_{n=1}^N \prod\limits_{t=1}^{T-1} \left[\sum_{i\in\mathcal{V}}\sum_{j\in dpa_d(i)}X^{(n)}_i(t+1) X^{(n)}_j(t)\theta^{d,i,j}+\sum_{i\in\mathcal{V}}\sum_{j\in dpa_s(i)}X^{(n)}_i(s+1) X^{(n)}_j(s+1)\theta^{s,i,j}\right.\\\qquad\qquad\left.+\sum_{i\in\mathcal{V}}\sum_{j\in dpa_z(i)}X^{(n)}_i(s+1) Z^{(n)}_j\theta^{z,i,j}+\sum_{i\in\mathcal{V}}\sum_{\tau\in [p]}X^{(n)}_i(s+1) X^{(n)}_i(s+1-\tau)\theta^{a,i,\tau}\right] \\
\qquad = 
\sum_{i\in\mathcal{V}}\sum_{j\in dpa_d(i)}  \left(\theta^{d,i,j}\right)^{N(t,n:X^{(n)}_j(t)\cap X^{(n)}_i(t-1))}\left(1-\theta^{d,i,j}\right)^{N(t,n:X^{(n)}_j(t)\cap (1-X^{(n)}_i(t-1)))}\\\qquad\qquad+\sum_{i\in\mathcal{V}}\sum_{j\in dpa_s(i)}\left(\theta^{s,i,j}\right)^{N(t,n:X^{(n)}_j(t)\cap X^{(n)}_i(t))}\left(1-\theta^{s,i,j}\right)^{N(t,n:X^{(n)}_j(t)\cap (1-X^{(n)}_i(t)))}\\\qquad\qquad+\sum_{i\in\mathcal{V}}\sum_{j\in dpa_z(i)}\left(\theta^{z,i,j}\right)^{N(t,n:X^{(n)}_j(t)\cap Z^{(n)}_i)}\left(1-\theta^{z,i,j}\right)^{N(t,n:(1-X^{(n)}_j(t))\cap Z^{(n)}_i)} \\ 
\qquad\qquad  
+\sum_{i\in\mathcal{V}}\sum_{\tau\in [p]}
\left(\theta^{a,i,\tau}\right)^{N(t,n:X^{(n)}_i(t-\tau)\cap X^{(n)}_i(t))}\left(1-\theta^{a,i,j}\right)^{N(t,n:(1-X^{(n)}_i(t))\cap X^{(n)}_i(t-\tau))}









Now we can see that the parameters are entirely sum-separable. We can maximize the likelihood by maximizing the log of each expression. We obtain, for, e.g. each $\theta_{d,i,j}$,
\[
\begin{array}{l}
\log p\left(\mathcal{S}\vert \theta_{d,i,j},\bar{\mathcal{G}} \right) = N(t,n:X^{(n)}_i(t)\cap X^{(n)}_j(t-1))\log \theta_{d,i,j}\\ \qquad 
+N(t,n: (1-X^{(n)}_i(t))\cap X^{(n)}_j(t-1)))\log(1-\theta_{d,i,j}) 
\end{array}
\]
Taking a derivative and solving for zero we obtain:
\[
\theta_{d,i,j} = \frac{N(t,n:X^{(n)}_i(t)\cap X^{(n)}_j(t-1))}{N(t,n:X^{(n)}_j(t-1))}
\]
for which the maximum likelihood can be calculated to be,
\[
\begin{array}{l}
\sum_{i\in\mathcal{V}}\sum_{j\in dpa_d(i)}  \left(\frac{N(t,n:X^{(n)}_i(t)\cap X^{(n)}_j(t-1))}{N(t,n:X^{(n)}_j(t-1))}\right)^{N(t,n:X^{(n)}_i(t)\cap X^{(n)}_j(t-1))}
\\ \qquad\qquad\times
\left(1-\frac{N(t,n:X^{(n)}_i(t)\cap X^{(n)}_j(t-1))}{N(t,n:X^{(n)}_j(t-1))}\right)^{N(t,n:X^{(n)}_j(t-1)\cap (1-X^{(n)}_i(t)))}\\\,+\sum_{i\in\mathcal{V}}\sum_{j\in dpa_s(i)}\left(\frac{N(t,n:X^{(n)}_j(t)\cap X^{(n)}_i(t))}{N(t,n:X^{(n)}_j(t))}\right)^{N(t,n:X^{(n)}_j(t)\cap X^{(n)}_i(t))}\\ \qquad\qquad\left(1-\frac{N(t,n:X^{(n)}_j(t)\cap X^{(n)}_i(t))}{N(t,n:X^{(n)}_j(t))}\right)^{N(t,n:X^{(n)}_j(t)\cap (1-X^{(n)}_i(t)))}\\\,+\sum_{i\in\mathcal{V}}\sum_{j\in dpa_z(i)}\left(\frac{N(t,n:X^{(n)}_i(t)\cap Z^{(n)}_j)}{N(t,n:X^{(n)}_i(t))}\right)^{N(t,n:X^{(n)}_i(t)\cap Z^{(n)}_j)}\\ \qquad\qquad\left(1-\frac{N(t,n:X^{(n)}_i(t)\cap Z^{(n)}_j)}{N(t,n:Z^{(n)}_j)}\right)^{N(t,n:(1-X^{(n)}_i(t))\cap Z^{(n)}_j)} 
\\\,+\sum_{i\in\mathcal{V}}\sum_{\tau\in [p]}\left(\frac{N(t,n:X^{(n)}_i(t)\cap X^{(n)}_i(t-\tau))}{N(t,n:X^{(n)}_i(t-\tau))}\right)^{N(t,n:X^{(n)}_i(t)\cap X^{(n)}_{i}(t-\tau))}\\ \qquad\qquad\left(1-\frac{N(t,n:X^{(n)}_i(t)\cap X^{(n)}_i(t-\tau))}{N(t,n:X^{(n)}_i(t-\tau))}\right)^{N(t,n:(1-X^{(n)}_i(t))\cap Z^{(n)}_j)} 
\end{array}
\]

%= \prod\limits_{n=1}^N \prod\limits_{s=1}^{T-1}\left[ 1-X_i^{(n)}(s)-P_{t,i}(\theta)+2P_{t,i}(\theta)X_i^{(n)}(s)\right]
One can then evaluate any of the criteria in the standard way~\eqref{eq:criterion}.











\sum_{\{(d,i,j)\}\cup\{s,i,j\}\cup\{z,i,j\}\cup\{s,i,\tau\}} \int_{\theta^{\bar{\mathcal{G}}}} P(\mathcal{S}|\theta^{\bar{\mathcal{G}}},\bar{\mathcal{G}})P(\theta^{\bar{\mathcal{G}}}|\bar{\mathcal{G}})d\theta \\
\\
\qquad = 
\sum_{i\in\mathcal{V}}\sum_{j\in dpa_d(i)}  
\int_{\theta^{d,i,j}} \left(\theta^{d,i,j}\right)^{\alpha_{d,i,j}+N(t,n:X^{(n)}_j(t)\cap X^{(n)}_i(t-1))}\left(1-\theta^{d,i,j}\right)^{N(t,n:X^{(n)}_j(t)\cap (1-X^{(n)}_i(t-1)))}d \theta^{d,i,j}\\\qquad\qquad+\sum_{i\in\mathcal{V}}\sum_{j\in dpa_s(i)}\int_{\theta^{s,i,j}} \left(\theta^{s,i,j}\right)^{\alpha_{s,i,j}+N(t,n:X^{(n)}_j(t)\cap X^{(n)}_i(t))}\left(1-\theta^{s,i,j}\right)^{N(t,n:X^{(n)}_j(t)\cap (1-X^{(n)}_i(t)))}d\theta^{s,i,j} \\\qquad\qquad+\sum_{i\in\mathcal{V}}\sum_{j\in dpa_z(i)}\int_{\theta^{z,i,j}}\left(\theta^{z,i,j}\right)^{\alpha_{z,i,j}+N(t,n:X^{(n)}_j(t)\cap Z^{(n)}_i)}\left(1-\theta^{z,i,j}\right)^{N(t,n:(1-X^{(n)}_j(t))\cap Z^{(n)}_i)} d \theta^{z,i,j}\\ 
\qquad\qquad 
+\sum_{i\in\mathcal{V}}\sum_{\tau\in [p]}\int_{\theta^{a,i,\tau}}
\left(\theta^{a,i,\tau}\right)^{\alpha_{i,\tau}+N(t,n:X^{(n)}_i(t-\tau)\cap X^{(n)}_i(t))}\left(1-\theta^{a,i,j}\right)^{N(t,n:(1-X^{(n)}_i(t))\cap X^{(n)}_i(t-\tau))}d \theta^{a,i,\tau}






Now the BDe can be computed to be:
\[
\begin{array}{l}
P(\mathcal{S}\vert \bar{\mathcal{G}}) = 
\prod\limits_{i\in[n]}
\prod\limits_{n=1}^N \prod\limits_{t=1}^{T-1} 
\int_{\theta^{\bar{\mathcal{G}}}}  
\left[
\mathbf{1}(X^{(n)}_i(t+1)=1)P(X^{(n)}_i(t+1)=1\vert V^{(n)}_{dpa(i)} ;\theta)
\right. \\ \qquad\qquad \left.+\mathbf{1}(X^{(n)}_i(t+1)=0)P(X^{(n)}_i(t+1)=0\vert V^{(n)}_{dpa(i)} ;\theta)\right]\prod_{j\in dpa(i)}\theta^{\alpha_{i,j}}
\end{array}
\]




\Sigma_d(1,0) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_i^{(n)}(1)-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(X_{j\in dpa_t(i)}^{(n')}(0)-\frac{1}{N}\sum_{m} X_{j\in dpa_t(i)}^{(m)}(0)\right)^T \\ 
\Sigma^{\nu}_d(1,0) = \frac{1}{N}\sum_{n}\left(\nu-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(X_{j\in dpa_t(i)}^{(n')}(0)-\frac{1}{N}\sum_{m} X_{j\in dpa_t(i)}^{(m)}(0)\right)^T \\ 
\Sigma_d(0,0) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_{j\in dpa_t(i)}^{(n')}(0)-\frac{1}{N}\sum_{m} X_{j\in dpa_t(i)}^{(m)}(0)\right)\left(X_{j\in dpa_t(i)}^{(n')}(0)-\frac{1}{N}\sum_{m} X_{j\in dpa_t(i)}^{(m)}(0)\right)^T
\\
\Sigma_s(1,0) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_i^{(n)}(1)-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(Z_{j\in dpa_z(i)}^{(n')}-\frac{1}{N}\sum_{m} Z_{j\in dpa_z(i)}^{(m)}\right)^T \\ 
\Sigma^{\nu}_s(1,0) = \frac{1}{N}\sum_{n}\left(\nu-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(Z_{j\in dpa_z(i)}^{(n')}-\frac{1}{N}\sum_{m} Z_{j\in dpa_z(i)}^{(m)}\right)^T \\ 
\Sigma_s(0,0) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(Z_{j\in dpa_z(i)}^{(n)}-\frac{1}{N}\sum_{m} Z_{j\in dpa_z(i)}^{(m)}(1)\right)\left(V_i^{(n')}(1)-\frac{1}{N}\sum_{m} Z_{j\in dpa_z(i)}^{(m)}\right)^T










































Let us now present the expression for one time step, considering the initialization as at $t=0$,
\begin{equation}\label{eq:bgeposterior}
\begin{array}{l}
p(W(1),\bar{\mathcal{G}}) = \text{Wishart}(W(1)\vert \alpha_w+N,T(1))\\
T(1)=T+\Sigma(1,1)+\frac{\alpha_{mu} N}{\alpha_{\mu}+N}\left\{ \Sigma^{\nu}(0,0)
- \Sigma^{\nu}(1,0)\Sigma^\nu(0,0)^{-1}\Sigma^{\nu}(1,0)^T \right\}\\
\Sigma(1,1) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_i^{(n)}(1)-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(X_i^{(n)}(1)-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)^T  \\
\Sigma^\nu(0,0) = \left(\chi(0)-\frac{1}{N}\sum_{m} V_i^{(m)}(1)\right)\left(\chi(0)-\frac{1}{N}\sum_{m} V_i^{(m)}(1)\right)^T  \\
\Sigma^\nu(1,0) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_i^{(n)}(1)-\nu_0+\frac{1}{N}\sum_{m} \nu_{\setminus 0} \cdot V_i^{(m)}(1)\right)\left(\chi(0)-\frac{1}{N}\sum_{m} V_i^{(m)}(1)\right)^T \\ 
\\
p\left(\mu_{i,0}\vert W(1),\mathcal{S}_{t=0,1},\bar{\mathcal{G}}\right)
= \mathcal{N}\left(\nu_0(1),(\alpha_{\mu}+N) \tilde{W}_0(1)\right),\\ 
\nu_0(1) = \frac{\alpha_{\mu}\nu_0 +\Sigma^{\nu}(1,0)\Sigma^\nu(0,0)^{-1}  \sum\limits_{n\in[N]} V_i^{(n)}(1)}
{\alpha_{\mu}+N} \\
p\left([\mu_d]_{i,j}\vert W(1),\mathcal{S}_{t=0,1},\bar{\mathcal{G}}\right)
= \mathcal{N}\left(\nu_d(1),(\alpha_{\mu}+N) \tilde{W}_{i;d;j}(1)\right), \\
\nu_d(1) = \frac{\alpha_{\mu}[\nu_d]_{i,j} + \Sigma_d(0,0)^{-1}(\Sigma_d(1,0)+\Sigma^{\nu}_d(1,0))}
{\alpha_{\mu}+N} \\
p\left([\mu_s]_{i,j}\vert W,\mathcal{S},\bar{\mathcal{G}}\right)
= \mathcal{N}\left(\nu_s(1),(\alpha_{\mu}+N) \tilde{W}_{i;s;j}(1)\right), \\ 
\nu_s(1) = \frac{\alpha_{\mu}[\nu_s]_{i,j} + \Sigma_s(0,0)^{-1}(\Sigma_s(1,0)+\Sigma_s^{\nu}(1,0)}
{\alpha_{\mu}+N} \\
\chi(1) = \{\frac{1}{N}\sum_{n\in[N]} X^{(n)}(1)\},\chi_z(0)\} 
\end{array}
\end{equation}
where we use $W_{w,\setminus}$ the cross diagonal components of the covariance matrix (that is, covariance between $v$ and all of the other quantities). Indices in $W$ correspond to parameter vector components, that is, $0$ for $\beta_0$, then $d$ and $s$ for the dynamic and static linear terms. Recall that $V^{(n)}_{j}(1)$ could be $Z^{(n)}_k$ for some $k$ or $X^{(n)}_k(0)$ for some $k$, it corresponds to the nodes that influence transitions to time one. 

We can see from these that since every time transition is Gaussian, with a known prior distribution, the posterior of the weight distribution is normal-Wishart. The prior knowledge and the data both influence all of the expressions. Now let us perform the recursion of this operation from $T-1$ to $T$:


Recall that
\[
\tilde{W}_{a}=W_{aa}-W_{a,\setminus} W_{\setminus,\setminus}^{-1} W_{\setminus,a}
\]
can be used to obtain the components with respect to a particular subset of parameters
%\[
%\begin{array}{l}p\left(\mu\vert W,\mathcal{S},\bar{\mathcal{G}}\right)
%= \mathcal{N}\left(\frac{\alpha_{\mu}\nu + \sum\limits_{n\in[N]} X^{(n)}(1)}
%{\alpha_{\mu}+N},(\alpha_{\mu}+N) W\right),\\
%\end{array}
%\]
%Observe that the expression $\sum\limits_{n\in[N]} X^{(n)}(1)$ corresponds to the sample mean of the data, and this estimate resembles the standard expression of the Bayesian model being maximum likelihood estimate perturbed with additive terms incorporating prior knowledge as corresponding to, effectively, additional samples. The posterior Covariance Matrix $W$ is now, conjugately, a Wishart distribution given by,
%\[
%\begin{array}{l}
%W \sim \text{Wishart}\left(W \vert a_w+N,T+\sum\limits_{n\in[N]} 
%\left(X^{(n)}(1)-\frac{1}{N}\sum_{l\in[N]} X^{(l)}(1)\right)
%\left(X^{(n)}(1)-\frac{1}{N}\sum_{l\in[N]} X^{(l)}(1)\right)^T\right.\\\qquad\qquad\left.+\frac{a_{\mu} N}{a_{\mu}+N}\left(\nu -\frac{1}{N}\sum_{l\in[N]} X^{(l)}(1)\right)
%\left(\nu-\frac{1}{N}\sum_{l\in[N]} X^{(l)}(1)\right)^T\right)^T
%\end{array}
%\]
%It is at this point that, unlike in the discrete case where the history presents itself simply as far as which nodes and time steps you count. In this case, in order to take into account the fact that the next transition takes place from a new instantiation of $X$, we have to include it explicitly.


Now, let us consider the inductive process, by which we can derive the expression for the posterior given the data through all of the time steps $T$. Indeed we can expect the same posterior updates, with an additional sample informing the mean and covariance of the Gaussian model in the same arithmetic manner each time step, and thus the derivation again resulting in a conjugate normal-Wishart distribution. 

From the expressions in~\eqref{eq:bgeposterior}, we can consider that the following terms can be defined analogously:
\[ 
\begin{array}{l}
\Sigma(t+1,t+1) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_i^{(n)}(t+1)-\frac{1}{N}\sum_{m} X_i^{(m)}(t+1)\right)\left(X_i^{(n)}(t+1)-\frac{1}{N}\sum_{m} X_i^{(m)}(t+1)\right)^T  \\
\Sigma^\nu(t+1,t+1) = \left(\nu(t)+\frac{1}{N}\sum_n \left(( X^{(n)}(t+1)-\frac{1}{N}\sum_{m} X_i^{(m)}(t+1)\right)\right)\\ \qquad\qquad\times \left(\nu+\frac{1}{Nt}\sum_s\sum_n \left(X^{(n)}(t+1)-\frac{1}{N}\sum_{m} X_i^{(m)}(t+1)\right)\right)^T  \\
\Sigma(t+1,t) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_i^{(n)}(t+1)-\frac{1}{N}\sum_{m} X_i^{(m)}(t+1)\right)\left(V_i^{(n')}(t+1)-\frac{1}{N}\sum_{m} V_i^{(m)}(t+1)\right)^T \\ 
\Sigma^{\nu}(t+1,t) = \frac{1}{N^2t}\sum_{n'}\sum_{\tilde{s} <s'}\left(\nu(t)+\frac{1}{N}\sum_{m} X_i^{(m)}(\tilde{s})-\frac{1}{N}\sum_{m} X_i^{(m)}(s'+1)\right)\left(V_i^{(n')}(s'+1)-\frac{1}{N}\sum_{m} V_i^{(m)}(s'+1)\right)^T \\ 
\Sigma(t,t) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(V_i^{(n)}(t+1)-\frac{1}{N}\sum_{m} V_i^{(m)}(t+1)\right)\left(V_i^{(n')}(t+1)-\frac{1}{N}\sum_{m} V_i^{(m)}(t+1)\right)^T
\\
\Sigma_d(t+1,t) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_i^{(n)}(1)-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(X_{j\in dpa_t(i)}^{(n')}(0)-\frac{1}{N}\sum_{m} X_{j\in dpa_t(i)}^{(m)}(0)\right)^T \\ 
\Sigma^{\nu}_d(t+1,t) = \frac{1}{N}\sum_{n}\left(\nu-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(X_{j\in dpa_t(i)}^{(n')}(0)-\frac{1}{N}\sum_{m} X_{j\in dpa_t(i)}^{(m)}(0)\right)^T \\ 
\Sigma_d(t,t) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_{j\in dpa_t(i)}^{(n')}(0)-\frac{1}{N}\sum_{m} X_{j\in dpa_t(i)}^{(m)}(0)\right)\left(X_{j\in dpa_t(i)}^{(n')}(0)-\frac{1}{N}\sum_{m} X_{j\in dpa_t(i)}^{(m)}(0)\right)^T
\\
\Sigma_s(t+1,t) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(X_i^{(n)}(1)-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(Z_{j\in dpa_z(i)}^{(n')}-\frac{1}{N}\sum_{m} Z_{j\in dpa_z(i)}^{(m)}\right)^T \\ 
\Sigma^{\nu}_s(t+1,t) = \frac{1}{N}\sum_{n}\left(\nu-\frac{1}{N}\sum_{m} X_i^{(m)}(1)\right)\left(Z_{j\in dpa_z(i)}^{(n')}-\frac{1}{N}\sum_{m} Z_{j\in dpa_z(i)}^{(m)}\right)^T \\ 
\Sigma_s(t,t) = \frac{1}{N^2}\sum_{n}\sum_{n'}\left(Z_{j\in dpa_z(i)}^{(n)}-\frac{1}{N}\sum_{m} Z_{j\in dpa_z(i)}^{(m)}(1)\right)\left(V_i^{(n')}(1)-\frac{1}{N}\sum_{m} Z_{j\in dpa_z(i)}^{(m)}\right)^T
\end{array}
\]
and the expressions for the general posterior can be given by:
\begin{equation}\label{eq:bgeposteriorT}
\begin{array}{l}
p(W(T),\bar{\mathcal{G}}) = \text{Wishart}(W(T)\vert \alpha_w+NT,T(T))\\
T(T)=T+\sum_{t=1}^T\Sigma(t,t)+\frac{\alpha_{mu} NT}{\alpha_{\mu}+NT}\sum_{t} \Sigma^{\nu}(t+1,t+1)
\\ 
\qquad\qquad\qquad -\sum_t\left(\Sigma(t+1,t)+\frac{\alpha_{mu} N}{\alpha_{\mu}+N} \Sigma^{\nu}(t+1,t)\right) \Sigma(t,t)^{-1}\left( \Sigma(t+1,t)+\frac{\alpha_{\mu} N}{\alpha_{\mu}+N} \Sigma^{\nu}(t+1,t)\right)^T \\
p\left(\mu_{i,0}\vert W(1),\mathcal{S},\bar{\mathcal{G}}\right)
= \mathcal{N}\left(\frac{\alpha_{\mu}\nu_0 +\frac{1}{NT}\sum\limits_{t\in[T]}\sum\limits_{n\in[N]} X^{(n)}_i(1)- \sum\limits_{t\in[T-1]}(\Sigma(t+1,t)+\Sigma^{\nu}(t+1,t))\Sigma(t,t)^{-1}  \sum\limits_{n\in[N]} V_i^{(n)}(t+1)}
{\alpha_{\mu}+NT},\right.\\ \qquad\qquad \left.(\alpha_{\mu}+NT) \tilde{W}_0(T)\right),\\ 
p\left([\mu_d]_{i,j}\vert W(T),\mathcal{S},\bar{\mathcal{G}}\right)
= \mathcal{N}\left(\frac{\alpha_{\mu}[\nu_d]_{i,j} + \sum_{t\in[T-1]}\Sigma_d(t,t)^{-1}(\Sigma_d(t+1,t)+\Sigma^{\nu}_d(t+1,t))}
{\alpha_{\mu}+NT},(\alpha_{\mu}+NT) \tilde{W}_{i;d;j}(T)\right), \\
p\left([\mu_s]_{i,j}\vert W,\mathcal{S},\bar{\mathcal{G}}\right)
= \mathcal{N}\left(\frac{\alpha_{\mu}[\nu_s]_{i,j} + \sum_[t\in[T-1]\Sigma_s(t,t)^{-1}(\Sigma_s(t+1,t)+\Sigma_s^{\nu}(t+1,t))
}{\alpha_{\mu}+NT},(\alpha_{\mu}+NT) \tilde{W}_{i;s;j}(T)\right), 
\end{array}
\end{equation}

Finally, we can obtain the marginal likelihood of a structure $\bar{\mathcal{G}}$ from (see equation (18))~\cite{geiger2002parameter}:























\subsection{Novel Modifications of Existing Methods}
In developing the work for this paper, a few natural developments of existing algorithms, that wouldn't be worthwhile to appear independently, arose. We present each of these methods and describe them 


\paragraph{One Shot Structure-Parameter Consistent Frequentist}

We propose a modified variant of~\eqref{eq:iposmod}. In this case, we introduce positive and negative weights, and require a lower bound for the weights. Thus, if the edge is active, the weights are forced to be bounded away from zero. This is based on two motivations:
\begin{enumerate}
    \item In principle, a structure being correctly identified should correspond to the weights associated with any active edge to be nonzero. Thus a search for the structure fitting the data well should be expected to have weights that would reject a null hypothesis of zero. 
    \item In the literature on sparsity ($\|\cdot\|_0$) constrained optimization, e.g.~\cite{beck2016minimization}, it can be seen that a necessary (but not sufficient) condition for optimality is an $L$-stationarity condition that implies that, effectively, the indices $\mathcal{I}(\theta^*)=\mathop{supp}(\theta^*)$ are such that $\theta_i,i\in\mathcal{I}(\theta^*)$ must be bounded away from zero a distance corresponding the Lipschitz constant of the gradient and the gradient vector components corresponding to the components of $\theta^*$ that are zero. 
\end{enumerate}




\begin{equation}\label{eq:iposmod}
    \begin{array}{rl}
\min\limits_{\left(\begin{array}{c}E_{W^+},E_{W^-},E_{A^+},E_{A^-} \\ W^{+},W^{-},A^{+},A^{-}\end{array}\right)} & \mathbf{E}((E_{W^+},E_{W^-},E_{A^+},E_{A^-},W^{+},W^{-},A^{+},A^{-}))\\ & 
+\lambda_{W^+} \|E_{W^+}\|_0+\lambda_{W^-} \|E_{W^-}\|_0+\lambda_{A^+}\|E_{A^+}\|_0+ \lambda_{A^-}\|E_{A^-}\|_0
\\ &:=\sum\limits_{m=1}^M\sum\limits_{t=1}^T\sum\limits_{i=1}^d\left([X_{m,t}]_i-\sum\limits_{j=1}^d [E_{W^+}]_{l,j,i}W^+_{j,i}[X_{m,t}]_j
-\sum\limits_{j=1}^d [E_{W^-}]_{l,j,i}W^-_{j,i}[X_{m,t}]_j\right.\\&\left.-\sum\limits_{l=1}^{\min\{p,t\}}\sum\limits_{j=1}^n [E_{A^+}]_{l,j,i}A^+_{l,j,i} [X_{m,t-l}]_j-\sum\limits_{l=1}^{\min\{p,t\}}\sum\limits_{j=1}^n [E_{A^-}]_{l,j,i}A^-_{l,j,i} [X_{m,t-l}]_j\right)^2 \\ & +\lambda_{W^+} \sum\limits_{i,j} [E_{W^+}]_{i,j}
+\lambda_{W^-} \sum\limits_{i,j} [E_{W^-}]_{i,j} \\ &
+\lambda_{A^+}\sum\limits_{l,i,j}[E_{A^+}]_{l,i,j}
+\lambda_{A^-}\sum\limits_{l,i,j}[E_{A^-}]_{l,i,j}\\
\text{s.t. } &  W^{+}\ge  b_W,\, W^- \le - b_W\\
& A^+\ge b_A, \, A^- \le - b_A\\
& E_{W^+}+E_{W^-}\le 1,\, E_{A^+}+E_{A^-}\le 1 \\
%& W^+\cdot (1-E_{W^+})=0,\,W^-\cdot (1-E_{W^-})=0\\
%& A^+\cdot (1-E_{A^+})=0,\,A^-\cdot (1-E_{A^-})=0\\
& DAG\left(E_{W^+}+E_{W^-}\right), \\
& E_{W^+},E_{W^-}\in \left[\{0,1\}^{d^2}\right]\\
& E_{A^+},E_{A^-} \in \left[\{0,1\}^{d^2}\right]^p \\
& W^+,W^-\in\mathbb{R}^{d\times d},\, A^+,A^-\in\mathbb{R}^{p\times d\times d}
    \end{array}
\end{equation}
where $b_W,b_A>0$ are lower bounds on the magnitude of these weights.


